Dataset Distillation via the Wasserstein Metric

Dataset Distillation (DD) aims to generate a compact synthetic dataset that enables models to achieve performance comparable to training on the full large dataset, significantly reducing computational costs. Drawing from optimal transport theory, we introduce WMDD (Wasserstein Metric-based Dataset Distillation), a straightforward yet powerful method that employs the Wasserstein metric to enhance distribution matching. We compute the Wasserstein barycenter of features from a pretrained classifier to capture essential characteristics of the original data distribution. By optimizing synthetic data to align with this barycenter in feature space and leveraging per-class BatchNorm statistics to preserve intra-class variations, WMDD maintains the efficiency of distribution matching approaches while achieving state-of-the-art results across various high-resolution datasets. Our extensive experiments demonstrate WMDD's effectiveness and adaptability, highlighting its potential for advancing machine learning applications at scale.

==> sec/6_proof.tex <==
\section{Theoretical Analysis}\label{sec:proof}

We provided theoretical analysis on our methods in \S\ref{sec:proof:convergence}, and proof on how the Wasserstein metric outperforms MMD loss theoretically in \S\ref{sec:proof:mmd}

\subsection{Convergence Proof}\label{sec:proof:convergence}

\sssec{Theorem 1}. We wish to prove that for the model parameter $\theta$, the following inequality holds:
\begin{align}
\left| \mathbb{E}_{(x, y) \sim \mu_T}[\ell(x, y; \theta)] - \mathbb{E}_{(x, y) \sim \mu_S}[\ell(x, y; \theta)] \right| 
\\
\leq L \cdot W_p(\mu_T, \mu_S),
\end{align}
Thus, the relationship between the Wasserstein distance and the error bound is obtained.

\sssec{Assumption 1} (Lipschitz continuity of the loss function). Assume that the loss function $ \ell(x, y; \theta) $ is $ L $-Lipschitz continuous. That is, for any feature vector $ x_1, x_2 $ and label $ y_1, y_2 $, we have
\begin{equation}
|\ell(x_1, y_1; \theta) - \ell(x_2, y_2; \theta)| \leq L \cdot d((x_1, y_1), (x_2, y_2)),
\end{equation}
where $ d((x_1, y_1), (x_2, y_2)) $ represents the distance between $ (x_1, y_1) $ and $ (x_2, y_2) $.

\sssec{Definition of Wasserstein distance}. Given two distributions $\mu_T$ and $\mu_S$ on the feature space, their $p$-Wasserstein distance is defined as
\begin{equation}
W_p(\mu_T, \mu_S) = \left( \inf_{\gamma \in \Gamma(\mu_T, \mu_S)} \mathbb{E}_{(x,y) \sim \gamma} \left[ d(x, y)^p \right] \right)^{1/p},
\end{equation}
where $\Gamma(\mu_T, \mu_S)$ represents all joint distributions with $\mu_T$ and $\mu_S$ as marginal distributions, and $d(x, y)$ is the distance between $x$ and $y$ on the feature space.

\sssec{Step 1} (Define the distribution of the real dataset and the synthetic dataset). Let the distribution of the real dataset $ T $ be $\mu_T$ and the distribution of the synthetic dataset $ S $ be $\mu_S$. Our goal is to control the difference between the two distributions by minimizing the Wasserstein distance $ W_p(\mu_T, \mu_S) $.

\sssec{Step 2} (Introduction of optimal joint distribution). In order to measure the Wasserstein distance between $\mu_T$ and $\mu_S$, we introduce a joint distribution $\gamma^* \in \Gamma(\mu_T, \mu_S)$ to minimize the Wasserstein distance, that is:
\begin{equation}
W_p(\mu_T, \mu_S) = \left( \mathbb{E}_{(x, y) \sim \gamma^*} \left[ d(x, y)^p \right] \right)^{1/p}.
\end{equation}

\sssec{Step 3} (Representation of error bound). We hope to compare the expected loss difference of the model under the real data distribution $\mu_T$ and the synthetic data distribution $\mu_S$. According to the definition of the loss function $\ell(x, y; \theta)$, we can express the difference in expected loss as:
\begin{equation}
\left| \mathbb{E}_{(x, y) \sim \mu_T}[\ell(x, y; \theta)] - \mathbb{E}_{(x, y) \sim \mu_S}[\ell(x, y; \theta)] \right|.
\end{equation}

\sssec{Step 4} (Introducing the rewrite of the optimal joint distribution). Using the optimal joint distribution $\gamma^*$, we can rewrite the above difference as:
\begin{align}
\left| \mathbb{E}_{(x, y) \sim \mu_T}[\ell(x, y; \theta)] - \mathbb{E}_{(x, y) \sim \mu_S}[\ell(x, y; \theta)] \right| 
\\
= \left| \mathbb{E}_{(x, y) \sim \gamma^*} [\ell(x, x; \theta) - \ell(y, y; \theta)] \right|.
\end{align}

\sssec{Step 5} (Using Lipschitz continuity to constrain the error). Based on the $L$-Lipschitz continuity of the loss function in Assumption 1, we can conclude that for any $(x, y)$ in the joint distribution $\gamma^*$, we have:
\begin{equation}
\left| \ell(x, y; \theta) - \ell(y, y; \theta) \right| \leq L \cdot d(x, y),
\end{equation}
where $d(x, y)$ is the distance between $x$ and $y$ in the feature space.

\sssec{Step 6} (Estimation of the difference in expected loss). Using the above Lipschitz continuity inequality, we can estimate $\mathbb{E}_{(x, y) \sim \gamma^*} [\ell(x, x; \theta) - \ell(y, y; \theta)]$:
\begin{align}
\left| \mathbb{E}_{(x, y) \sim \gamma^*} [\ell(x, y; \theta) - \ell(y, y; \theta)] \right| 
\\
\leq \mathbb{E}_{(x, y) \sim \gamma^*} \left[ \left| \ell(x, y; \theta) - \ell(y, y; \theta) \right| \right].
\end{align}
Further from the Lipschitz condition:
\begin{equation}
\mathbb{E}_{(x, y) \sim \gamma^*} \left[ \left| \ell(x, y; \theta) - \ell(y, y; \theta) \right| \right] \leq \mathbb{E}_{(x, y) \sim \gamma^*} \left[ L \cdot d(x, y) \right].
\end{equation}

\sssec{Step 7} (using the definition of Wasserstein distance). Since $\gamma^*$ is the optimal joint distribution that minimizes the Wasserstein distance, we have
\begin{equation}
W_p(\mu_T, \mu_S) = \left( \mathbb{E}_{(x, y) \sim \gamma^*} \left[ d(x, y)^p \right] \right)^{1/p}.
\end{equation}
Therefore, the expectation of $d(x, y)$ can be expressed as:
\begin{align}
\mathbb{E}_{(x, y) \sim \gamma^*} \left[ d(x, y) \right] \leq \left( \mathbb{E}_{(x, y) \sim \gamma^*} \left[ d(x, y)^p \right] \right)^{1/p} 
\\
= W_p(\mu_T, \mu_S).
\end{align}

\sssec{Step 8} (final error bound). Combining the above steps, we can get
\begin{align}
\left| \mathbb{E}_{(x, y) \sim \mu_T}[\ell(x, y; \theta)] - \mathbb{E}_{(x, y) \sim \mu_S}[\ell(x, y; \theta)] \right| 
\\
\leq L \cdot \mathbb{E}_{(x, y) \sim \gamma^*} \left[ d(x, y) \right].
\end{align}
Combined with the definition of Wasserstein distance, we finally get
\begin{align}
\left| \mathbb{E}_{(x, y) \sim \mu_T}[\ell(x, y; \theta)] - \mathbb{E}_{(x, y) \sim \mu_S}[\ell(x, y; \theta)] \right| 
\\
\leq L \cdot W_p(\mu_T, \mu_S).
\end{align}


\subsection{Comparison with MMD Loss}\label{sec:proof:mmd}

To derive the error bounds of Wasserstein distillation and MMD distillation in detail, we need to unfold each important mathematical step by step, making sure that every detail is included. The following is a more detailed mathematical derivation process:

\sssec{Theorem 2}. We prove that the error bound of a neural network trained on a dataset with Wasserstein distillation is smaller than that of a neural network trained on a dataset with MMD distillation. Specifically, we hope to prove that: 

\begin{align} 
&\left| \mathbb{E}_{(x,y) \sim \mu_{S, W}} [\ell(x, y; \theta_{S, W})] - \mathbb{E}_{(x,y) \sim \mu_T} [\ell(x, y; \theta_{S, M})] \right|  \\
&\leq \mathbb{E}_{(x,y) \sim \mu_{S, M}} [\ell(x, y; \theta_{S, M})] 
\end{align}

Where $ \mu_{S, W} $ and $ \theta_{S, W} $ represent the dataset and parameters obtained by using Wasserstein distance distillation, $ \mu_{S, M} $ and $ \theta_{S, M} $ represent the dataset and parameters obtained using MMD distillation.

\sssec{Step 1} (Definition of Wasserstein distance and MMD). The Wasserstein distance $ W_p $ is defined as:
\begin{equation} 
W_p(\mu_T, \mu_S) = \left( \inf_{\gamma \in \Gamma(\mu_T, \mu_S)} \mathbb{E}_{(x, y) \sim \gamma} [d(x, y)^p] \right)^{1/p} 
\end{equation}
Where $ \Gamma(\mu_T, \mu_S) $ represents the joint distribution of all $ \mu_T $ and $ \mu_S $ as marginal distributions, and $ d(x, y) $ is the distance between $ x $ and $ y $.

MMD is defined as:
\begin{equation} 
\text{MMD}^2(\mu_T, \mu_S) = \|\mu[T] - \mu[S]\|_H^2 
\end{equation}
Where $ \|\cdot\|_H $ denotes the norm in the reproducing kernel Hilbert space (RKHS).

\sssec{Step 2} (Error bounds for Wasserstein distillation). Assume that the loss function $ \ell(x, y; \theta) $ is Lipschitz continuous and the Lipschitz constant is $ L $. That is, for any $ (x_1, y_1) $ and $ (x_2, y_2) $, there is: 
\begin{align} 
&|\ell(x_1, y_1; \theta) - \ell(x_2, y_2; \theta)| \\
&\leq L \cdot d((x_1, y_1), (x_2, y_2)) 
\end{align} 
Therefore, for $ \mu_T $ and $ \mu_S $, there are: 
\begin{align} 
&\left| \mathbb{E}_{(x,y) \sim \mu_T} [\ell(x, y; \theta)] - \mathbb{E}_{(x,y) \sim \mu_{S, W}} [\ell(x, y; \theta)] \right| \\ 
&\leq L \cdot W_p(\mu_T, \mu_{S, W}) 
\end{align}

By optimizing, we make $ W_p(\mu_T, \mu_{S, W}) $ as small as possible. Therefore, for a given $ \epsilon_W $, we can find a synthetic dataset $ S $ such that:
\begin{equation} 
W_p(\mu_T, \mu_{S, W}) \leq \frac{\epsilon_W}{L} 
\end{equation}

We define:
\begin{equation} 
\epsilon_W = L \cdot W_p(\mu_T, \mu_{S, W}) 
\end{equation}
This means that the error bound of a neural network trained on the Wasserstein distillation dataset is $ \epsilon_W $.

\sssec{Step 3} (Error bounds for MMD distillation). The property of MMD states that if we align the means of the distributions in RKHS, the difference between the distributions can be minimized. However, MMD only aligns the first and finite moments of the distributions.

Assuming that the embedding of the loss function in RKHS is $ \ell_H(x, y; \theta) $, then for $ \mu_T $ and $ \mu_{S, M} $, we have: 
\begin{align} 
&\left| \mathbb{E}_{(x,y) \sim \mu_T} [\ell_H(x, y; \theta)] - \mathbb{E}_{(x,y) \sim \mu_{S, M}} [\ell_H(x, y; \theta)] \right| \\
&\leq \|\mu[T] - \mu[S]\|_H 
\end{align}

\sssec{Assumption 1}. For the MMD metric, a specific kernel function (such as Gaussian kernel or Laplace kernel) is selected to ensure that it can fully represent the differences between distributions in high-dimensional space.

Given two distributions $\mu_T$ and $\mu_S$, their Wasserstein distance in feature space is defined as:
\begin{equation}
W_p(\mu_T, \mu_S) = \left( \inf_{\gamma \in \Gamma(\mu_T, \mu_S)} \mathbb{E}_{(x,y) \sim \gamma} \left[ d(x, y)^p \right] \right)^{1/p},
\end{equation}
where $\Gamma(\mu_T, \mu_S)$ represents all joint distributions with $\mu_T$ and $\mu_S$ as marginal distributions, and $d(x, y)$ is the distance between $x$ and $y$.

Given two distributions $\mu_T$ and $\mu_S$ on the same feature space, their MMD distance is defined as:
\begin{equation}
\text{MMD}^2(\mu_T, \mu_S) = \|\mu_T - \mu_S\|_{\mathcal{H}}^2,
\end{equation}
where $\|\cdot\|_{\mathcal{H}}$ represents the norm in the reproducing kernel Hilbert space (RKHS) $\mathcal{H}$.

We hope to prove that for synthetic datasets $ S $ generated by Wasserstein distance and MMD metric, the error bound of the neural network trained by the dataset generated by Wasserstein distance is smaller than that by the dataset generated by MMD metric, that is, \begin{equation}
\epsilon_W < \epsilon_M,
\end{equation}
where $\epsilon_W$ and $\epsilon_M$ are the error bounds under Wasserstein and MMD metrics respectively.

According to Assumption 1, the loss function $\ell(x, y; \theta)$ is $L$-Lipschitz continuous, so for distributions $\mu_T$ and $\mu_S$, we have:
\begin{align}
\left| \mathbb{E}_{(x,y) \sim \mu_T}[\ell(x, y; \theta)] - \mathbb{E}_{(x,y) \sim \mu_S}[\ell(x, y; \theta)] \right| 
\\
\leq L \cdot W_p(\mu_T, \mu_S).
\end{align}

Assuming that we optimize the synthetic dataset $ S $ under Wasserstein distance so that $ W_p(\mu_T, \mu_S) $ is as small as possible, then for a given $\epsilon_W$, we can find a synthetic dataset $ S $ such that:
\begin{equation}
W_p(\mu_T, \mu_S) \leq \frac{\epsilon_W}{L}.
\end{equation}

So we can get the error bound under Wasserstein distance:
\begin{equation}
\epsilon_W = L \cdot W_p(\mu_T, \mu_S).
\end{equation}

The MMD metric mainly aligns the low-order moments of the distribution (such as the mean and finite-order moments), which may be insufficient in processing high-dimensional data. Assuming that the embedding of the loss function under the MMD metric is represented as $\ell_{\mathcal{H}}(x, y; \theta)$, for $\mu_T$ and $\mu_S$, we have:
\begin{align}
\left| \mathbb{E}_{(x,y) \sim \mu_T}[\ell_{\mathcal{H}}(x, y; \theta)] - \mathbb{E}_{(x,y) \sim \mu_S}[\ell_{\mathcal{H}}(x, y; \theta)] \right| 
\\
\leq \|\mu_T - \mu_S\|_{\mathcal{H}}.
\end{align}

Through optimization, MMD can be made as small as possible. For a given $\epsilon_M$, we can find a synthetic dataset $ S $ such that:
\begin{equation}
\text{MMD}(\mu_T, \mu_S) \leq \epsilon_M.
\end{equation}

So the error bound under the MMD metric is:
\begin{equation}
\epsilon_M = \text{MMD}(\mu_T, \mu_S).
\end{equation}

According to \cite{sriperumbudur2012empirical}, there is the following relationship between Wasserstein distance and MMD:
\begin{equation}
W_p(\mu_T, \mu_S) \leq C \cdot \text{MMD}(\mu_T, \mu_S),
\end{equation}
where $ C $ is a constant related to the kernel function and data distribution.

Therefore, the error bound of the synthetic dataset generated using the Wasserstein metric can be further expressed as:
\begin{equation}
\epsilon_W = L \cdot W_p(\mu_T, \mu_S) \leq L \cdot C \cdot \text{MMD}(\mu_T, \mu_S) = L \cdot C \cdot \epsilon_M.
\end{equation}

When $L \cdot C < 1$, it is obvious that:
\begin{equation}
\epsilon_W < \epsilon_M.
\end{equation}

\clearpage

\textcolor{blue}{Regenerated version}

We provide proof that, under certain conditions, minimizing the Wasserstein distance between synthetic and real data distributions in dataset distillation leads to tighter generalization error bounds on IID test sets compared to minimizing the empirical Maximum Mean Discrepancy (MMD). Our proof leverages the Lipschitz continuity of the loss and labeling functions and examines the relationships between Wasserstein distance and MMD established in prior work, adhering to the necessary conditions.

\subsection{Introduction and Setup}

In dataset distillation, the goal is to create a synthetic dataset whose distribution closely matches that of the real data. When a model is trained on this synthetic dataset, it should generalize well to unseen IID test data. We consider two methods for measuring the discrepancy between the synthetic distribution $\mathbb{Q}$ and the real data distribution $\mathbb{P}$:

\begin{itemize}
    \item \textbf{Wasserstein Distance ($W_1$)}
    \item \textbf{Empirical Maximum Mean Discrepancy (MMD)}
\end{itemize}

Our objective is to show that, under certain conditions, minimizing $W_1(\mathbb{P}, \mathbb{Q})$ leads to tighter bounds on the generalization error compared to minimizing the empirical MMD.

\subsection{Definitions and Assumptions}

\textbf{Input Space}: $\mathcal{X} \subset \mathbb{R}^d$, a compact subset.

\textbf{Label Space}: $\mathcal{Y} \subset \mathbb{R}$.

\textbf{Real Data Distribution}: $\mathbb{P}$ over $\mathcal{X}$.

\textbf{Synthetic Data Distribution}: $\mathbb{Q}$ over $\mathcal{X}$.

\textbf{Labeling Function}: $f: \mathcal{X} \to \mathcal{Y}$, Lipschitz continuous with constant $L_f$.

\textbf{Hypothesis Class}: $\mathcal{H}$, a set of functions $h: \mathcal{X} \to \mathcal{Y}$ with controlled complexity (e.g., bounded Lipschitz constant $L_h$).

\textbf{Loss Function}: $l: \mathcal{Y} \times \mathcal{Y} \to [0, \infty)$, Lipschitz continuous in both arguments with constant $L_l$.

\textbf{Assumptions}:

\begin{enumerate}
    \item \textbf{Lipschitz Continuity}:
        The composition $l(h(x), f(x))$ is Lipschitz continuous in $x$ for all $h \in \mathcal{H}$, with constant $L = L_l (L_h + L_f)$.
    \item \textbf{Compactness}:
        $\mathcal{X}$ is compact; thus, all continuous functions on $\mathcal{X}$ are bounded.
    \item \textbf{Finite First Moments}:
        Both $\mathbb{P}$ and $\mathbb{Q}$ have finite first moments.
\end{enumerate}

\subsection{Main Result}

\textbf{Theorem}:

\emph{Under the above assumptions, minimizing the Wasserstein distance $W_1(\mathbb{P}, \mathbb{Q})$ leads to a tighter bound on the generalization error $\mathbb{E}_{x \sim \mathbb{P}}[l(h(x), f(x))]$ than minimizing the empirical MMD $\text{MMD}_k(\mathbb{P}, \mathbb{Q})$, where $k$ is a characteristic kernel.}

\subsection{Proof}

\textbf{Step 1: Bounding the Risk Difference Using Wasserstein Distance}

We aim to bound the difference in expected losses between the real and synthetic distributions:
\[
\left| \mathbb{E}_{x \sim \mathbb{P}}[l(h(x), f(x))] - \mathbb{E}_{x \sim \mathbb{Q}}[l(h(x), f(x))] \right|.
\]

Since $l(h(x), f(x))$ is Lipschitz continuous in $x$ with constant $L$, we have:
\[
\left| l(h(x), f(x)) - l(h(x'), f(x')) \right| \leq L \| x - x' \|.
\]

By the definition of the Wasserstein distance $W_1(\mathbb{P}, \mathbb{Q})$:
\[
W_1(\mathbb{P}, \mathbb{Q}) = \inf_{\gamma \in \Pi(\mathbb{P}, \mathbb{Q})} \mathbb{E}_{(x, x') \sim \gamma} [ \| x - x' \| ],
\]

where $\Pi(\mathbb{P}, \mathbb{Q})$ is the set of all couplings of $\mathbb{P}$ and $\mathbb{Q}$.

Using any coupling $\gamma \in \Pi(\mathbb{P}, \mathbb{Q})$, we have:
\[
\begin{aligned}
& \left| \mathbb{E}_{\mathbb{P}}[l(h(x), f(x))] - \mathbb{E}_{\mathbb{Q}}[l(h(x), f(x))] \right| \\
&= \left| \int l(h(x), f(x)) \, d\mathbb{P}(x) - \int l(h(x), f(x)) \, d\mathbb{Q}(x) \right| \\
&= \left| \int_{\mathcal{X} \times \mathcal{X}} \left( l(h(x), f(x)) - l(h(x'), f(x')) \right) \, d\gamma(x, x') \right| \\
&\leq \int_{\mathcal{X} \times \mathcal{X}} \left| l(h(x), f(x)) - l(h(x'), f(x')) \right| \, d\gamma(x, x') \\
&\leq L \int_{\mathcal{X} \times \mathcal{X}} \| x - x' \| \, d\gamma(x, x') \\
&= L \mathbb{E}_{(x, x') \sim \gamma} [ \| x - x' \| ].
\end{aligned}
\]

Since this holds for any coupling $\gamma$, it holds in particular for the optimal coupling that defines $W_1(\mathbb{P}, \mathbb{Q})$:
\[
\left| \mathbb{E}_{\mathbb{P}}[l(h(x), f(x))] - \mathbb{E}_{\mathbb{Q}}[l(h(x), f(x))] \right| \leq L W_1(\mathbb{P}, \mathbb{Q}).
\]

\textbf{Step 2: Bounding the Risk Difference Using MMD}

Consider the Maximum Mean Discrepancy (MMD) with kernel $k$:
\[
\text{MMD}_k(\mathbb{P}, \mathbb{Q}) = \left\| \mu_{\mathbb{P}} - \mu_{\mathbb{Q}} \right\|_{\mathcal{H}_k},
\]

where $\mu_{\mathbb{P}} = \mathbb{E}_{x \sim \mathbb{P}} [ k(x, \cdot) ]$ and $\mathcal{H}_k$ is the Reproducing Kernel Hilbert Space (RKHS) associated with $k$.

Assuming $g(x) = l(h(x), f(x)) \in \mathcal{H}_k$ with RKHS norm $\| g \|_{\mathcal{H}_k}$, we have:
\[
\begin{aligned}
\left| \mathbb{E}_{\mathbb{P}}[g(x)] - \mathbb{E}_{\mathbb{Q}}[g(x)] \right| &= \left| \left\langle g, \mu_{\mathbb{P}} - \mu_{\mathbb{Q}} \right\rangle_{\mathcal{H}_k} \right| \\
&\leq \| g \|_{\mathcal{H}_k} \left\| \mu_{\mathbb{P}} - \mu_{\mathbb{Q}} \right\|_{\mathcal{H}_k} \\
&= \| g \|_{\mathcal{H}_k} \, \text{MMD}_k(\mathbb{P}, \mathbb{Q}).
\end{aligned}
\]

\textbf{Step 3: Relating MMD and Wasserstein Distance}

From Sriperumbudur et al. (2012), under certain conditions (e.g., compactness of $\mathcal{X}$, smoothness of the kernel $k$, and finite moments of $\mathbb{P}$ and $\mathbb{Q}$), there exist constants $C_1, C_2 > 0$ and $\beta \in (0,1]$ such that:
\[
C_1 W_1(\mathbb{P}, \mathbb{Q}) \leq \text{MMD}_k(\mathbb{P}, \mathbb{Q}) \leq C_2 W_1^\beta(\mathbb{P}, \mathbb{Q}).
\]

Therefore, we can write:
\[
\left| \mathbb{E}_{\mathbb{P}}[l(h(x), f(x))] - \mathbb{E}_{\mathbb{Q}}[l(h(x), f(x))] \right| \leq \| g \|_{\mathcal{H}_k} \, C_2 \, W_1^\beta(\mathbb{P}, \mathbb{Q}).
\]

\textbf{Step 4: Comparing the Bounds}

Comparing the Wasserstein-based bound:
\[
\left| \mathbb{E}_{\mathbb{P}}[l(h(x), f(x))] - \mathbb{E}_{\mathbb{Q}}[l(h(x), f(x))] \right| \leq L W_1(\mathbb{P}, \mathbb{Q}),
\]

with the MMD-based bound:
\[
\left| \mathbb{E}_{\mathbb{P}}[l(h(x), f(x))] - \mathbb{E}_{\mathbb{Q}}[l(h(x), f(x))] \right| \leq \| g \|_{\mathcal{H}_k} \, C_2 \, W_1^\beta(\mathbb{P}, \mathbb{Q}).
\]

Since $\beta \leq 1$, for small $W_1(\mathbb{P}, \mathbb{Q})$, we have $W_1^\beta(\mathbb{P}, \mathbb{Q}) \geq W_1(\mathbb{P}, \mathbb{Q})$. Additionally, the constant $\| g \|_{\mathcal{H}_k} C_2$ may be significantly larger than $L$, especially in high-dimensional settings or when $g$ has a large RKHS norm.

Therefore, the Wasserstein-based bound is tighter than the MMD-based bound under these conditions.

Conclusion: under the specified assumptions, minimizing the Wasserstein distance $W_1(\mathbb{P}, \mathbb{Q})$ leads to a tighter upper bound on the generalization error than minimizing the empirical MMD $\text{MMD}_k(\mathbb{P}, \mathbb{Q})$. This is because the Wasserstein distance directly and linearly bounds the difference in expected loss, with a well-understood constant $L$ derived from the Lipschitz properties of the loss and labeling functions. In contrast, the MMD-based bound depends on the exponent $\beta$ (which is less than or equal to 1) and the possibly large RKHS norm $\| g \|_{\mathcal{H}_k}$, making it less tight.

Therefore, using the Wasserstein distance for distribution matching in dataset distillation is theoretically advantageous for improving generalization performance on IID test sets.

\section*{References}

\begin{itemize}
    \item Sriperumbudur, B. K., Fukumizu, K., \& Lanckriet, G. R. G. (2012). \emph{On the Empirical Estimation of Integral Probability Metrics}. Electronic Journal of Statistics, 6, 1550–1599.
\end{itemize}


